Extremal Mechanisms for Pointwise Maximal Leakage

Data publishing under privacy constraints can be achieved with mechanisms that add randomness to data points when released to an untrusted party, thereby decreasing the data's utility. In this paper, we analyze this privacy-utility tradeoff for the pointwise maximal leakage privacy measure and a general class of convex utility functions. Pointwise maximal leakage (PML) was recently proposed as an operationally meaningful privacy measure based on two equivalent threat models: An adversary guessing a randomized function and an adversary aiming to maximize a general gain function. We study the behavior of the randomized response mechanism designed for local differential privacy under different prior distributions of the private data. Motivated by the findings of this analysis, we derive several closed-form solutions for the optimal privacy-utility tradeoff in the presented PML context using tools from convex analysis. Finally, we present a linear program that can compute optimal mechanisms for PML in a general setting.

==> sections/generalmechanisms.tex <==
In this Section, we provide an algorithmic solution for deriving mechanisms that are optimal in all privacy regions for uniform priors. Further, the proposed algorithm can be used to compute approximate solutions to the mechanism design problem in the case of non-uniform priors. The procedure is based on an important intuition about the PML privacy regions according to Definition \ref{def:privacyregions} and their consequences for the structure of optimal mechanisms. Consider the following composition result from \citet{saeidian2023inferential}:
\begin{lemma}[{{\cite[Theorem 4, 1)]{pml}}}]
\label{lem:pmlcomposition}
    Suppose $\boldsymbol{P}_{Y|X}$ satisfies $\epsilon_1$-PML, and for all  $y \in \supp(P_Y)$, the mechanism $\boldsymbol{P}_{Z|X,Y=y}$ satisfies $\epsilon_2$-PML, where $\epsilon_1,\epsilon_2 \geq 0$. Then the mechanism $\boldsymbol{P}_{YZ|X}$  satisfies $\epsilon$-PML with $\epsilon=\epsilon_1  + \epsilon_2$.
\end{lemma}
Next, note that any $\epsilon$ in the low-privacy regime can be decomposed as 
\begin{equation}
    \epsilon = \epsilon^* + \epsilon^+ := \epsilon_{N-2}(P_X) + (\epsilon - \epsilon_{N-2}(P_X)) = \log\frac{N}{2} + (\epsilon - \log\frac{N}{2}),
\end{equation}
that is, the chosen $\epsilon^+$ denotes the leakage that $\epsilon$ allows for on top of the required leakage for the low-privacy regime. Note that, in general, we have
\begin{equation}
\label{eq:MIMLPML}
    I(X;Y) \leq \mathcal{L}(X\to Y) \leq \epsilon.
\end{equation} 
As shown in \cite{IssaMaxL}, the LHS inequality in \eqref{eq:MIMLPML} holds with equality iff the mechanism induces a \emph{singular distribution} \cite{altuug2014singulardistributions}. Thus, the optimal mechanism $\boldsymbol{P}_{Y|X}$ satisfying $\epsilon^*$-PML in the case of uniform priors and mutual information as utility is the \emph{singular mechanism}, that is, a mechanism inducing a such singular distribution in conjunction with the prior distribution. Further, the RHS of \eqref{eq:MIMLPML} holds iff all outcomes of $X$ have the same probability. Therefore, in the case of uniform priors, PML and maximal leakage are in fact equal and this singular mechanism yields $\ell(X\to y) = \mathcal{L}(X\to Y) = \epsilon^*$ for all $y \in \mathcal{Y}$. Intuitively, this mechanism optimally discloses the answer to the query ``is $X$ in $\{x_i,x_j\}$" for some pre-defined pairs of $x_i, x_j \in \mathcal{X}$. Once an adversary observes the outcome of the mechanism, she knows the two symbols that the outcome of $X$ belongs to, but does not have any information on which one of the two symbols is more likely. Now, consider a second mechanism $\boldsymbol{P}_{Z|X,Y=y}$ that, given that we know the pair of symbols the outcome of $X$ belongs to (that is, we know $Y=y$), randomizes optimally between these two symbols $\{x_i,x_j\}$ such that the leakage of this binary mechanism is $\epsilon^+$. Then, by Lemma \ref{lem:pmlcomposition}, the combined leakage of the mechanisms will be smaller than or equal to $\epsilon^* + \epsilon^+ = \epsilon$. For the  binary mechanism, the optimal solution is known from Section \ref{sec:optsol:subsec:binary}. Now, from the composition rules of mutual information, we know that
\begin{equation}
    I(X;Y,Z) = I(X;Y) + I(X;Z|Y).
\end{equation}
In other words, the mutual information of a joint release of $Y$ and $Z$ is equal to the mutual information we get from first releasing $Y$, then releasing $Z$ while already possessing all information offered by the release of $Y$. In the presented case, this means that the mutual information of some variable $W=YZ$ yields the same utility as first revealing the answer to the query ``which of the (predefined) pairings does $X$ belong to?", and then further using the remaining additional leakage $\epsilon^+$ to provide more information about which of the two symbols in the pair is more likely. Since we know the optimal mechanism for answering both of these queries, we can calculate the mutual information we get from this two-mechanism construction as
\begin{align}
    I(X;Y) + I(X;Z|Y) &= \underbrace{\log N - H_b\biggl(\frac{1}{2}\biggr)}_{\text{singular distribution, optimal for } \epsilon^*} + \underbrace{\log 2 - H_b\biggl(\frac{\e^{\epsilon^+}}{2}\biggr)}_{\text{optimal binary mechanism for } \epsilon^+} \\
    &= \log N - \log 2 + \log 2 - H_b\biggl(\frac{\e^{\epsilon-\log \frac{N}{2}}}{2}\biggr) \\
    &= \log N - H_b\biggl(\frac{\e^{\epsilon}}{N}\biggr),
\end{align}
that is, this construction provides the same bound as derived above. This fact provides insights into the  structures of optimal mechanisms: Evidently, given the privacy level and the alphabet size, for uniform priors, the optimal mechanisms can be composed of an answer to a query indicating that the outcome of $X$ belongs to a pre-defined subset (in this case, pairs) 
and an optimal mechanism with a lower alphabet size revealing more information about the probabilities of each symbol in the indicated subset. In other words, the second mechanism is designed to ``fill up the gap" between the leakage of indicating this subset and the specified privacy level. %While this is valuable intuition, using it to prove optimality is not as direct as it might seem. Since Lemma \ref{lem:pmlcomposition} only states the composition \emph{satisfies} $\epsilon$-PML, it does not guarantee that there could not be another mechanism with higher utility that does not compose in this specific way, but still satisfies $\epsilon$-PML. Nevertheless, the preceding derivations hint at a specific structure of optimal mechanisms that seem promising for making mechanism design more easily interpretable in future work. 
Now, consider again the derivations in Section \ref{sec:prelim} on the connection between the privacy regions and disclosure of subset membership. Clearly, if $\epsilon$ falls into the $i^{\text{th}}$ privacy region, a singular mechanism indicating subset membership to subsets of size $N-i+1$ satisfies $\epsilon$-PML. Further, any additional leakage $\epsilon^+$ allowed for by the specified privacy level will obey
\begin{equation}
    \epsilon^+  \coloneqq \epsilon - \epsilon_{N-i-1}(P_X) < \epsilon_{1}(P_X).
\end{equation}
That is, by this construction, $\epsilon^+$ is guaranteed to be in the high-privacy regime. Since the optimal mechanism for the high-privacy regime is known from Section \ref{sec:optsol:subsec:highprivacy}, the concept derived above for values of $\epsilon$ in the low-privacy regime can therefore be generalized for all values of $\epsilon \geq 0$. Algorithm \ref{alg:splittingAlgo} implements the described procedure. Here, the procedure $\textsc{Singular}(i+1,P_X)$ returns a singular mechanism inducing a singular joint distribution with support size $i+1$ given the prior distribution $P_X$. This mechanism can then be used to indicate the subset membership of each outcome of $X$. The procedure $\textsc{OptimalHighPrivacy}(\epsilon^+,\frac{P_X}{\sum_{j=1}^{i+1}P_X(x_j)})$ releases the remaining information allowed for by the specified privacy level by returning an optimal high-privacy mechanism as presented in Section \ref{sec:optsol:subsec:highprivacy}. As the mechanism is designed to privatize between the elements of a smaller subset, the prior probabilities of its input have to be scaled to yield a valid probability distribution. 

\begin{algorithm}[!t]
\DontPrintSemicolon
\caption{General mechanisms via privacy region partitioning for uniform priors}\label{alg:splittingAlgo}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Privacy parameter $\epsilon$, prior distribution $P_X$ in non-increasing order.}
\Output{Privatization mechanisms $\boldsymbol{P}_{Y|X}$, $\boldsymbol{P}_{Z|X,Y=y}$}
\For{j = $1$ to $N-1$}
    {
    $\epsilon_j \gets (-\log \sum_{k=1}^{j}P_X(x_j))$ 
    }
$\mathcal{E} \gets \{0,\epsilon_1, \dots, \epsilon_{N-1}\}$\;
$i \gets \underset{i:\,(\epsilon - \epsilon_i) \geq 0}{\argmin}(\mathcal{E})$\;
$\epsilon^+ \gets \epsilon - \epsilon_i$\;
$\boldsymbol{P}_{Y|X} \gets \textsc{Singular}(i+1,P_X)$\;
$\boldsymbol{P}_{Z|X,Y=y} \gets \textsc{OptimalHighPrivacy}(\epsilon^+,\frac{P_X}{\sum_{j=1}^{i+1}P_X(x_j)})$\;
\end{algorithm}

Fig. \ref{fig:splittingAlgo} compares the utility of the optimal mechanism and the release procedure by Algorithm \ref{alg:splittingAlgo} for a uniform prior distribution. Evidently, the procedure achieves the same utility for all values of $\epsilon$.

\begin{figure*}
    \normalsize
    \begin{subfigure}[b]{.49\textwidth}
        \centering
            \input{fig/compAlgo_utility}
            \caption{Uniform Priors}
        \end{subfigure}
        \begin{subfigure}[b]{.49\textwidth}
            \centering
            \input{fig/compAlgo_utility}
            \caption{\hl{Non-uniform priors \textbf{needs to be added!}}}
        \end{subfigure}
        \caption{Caption}
        \label{fig:splittingAlgo}
\end{figure*}
